The Physics Behind the CosmicWatch Desktop Muon Detectors

The CosmicWatch Desktop Muon Detector is a Massachusetts Institute of Technology (MIT) and Polish National Centre for Nuclear Research (NCBJ) based undergraduate-level physics project that incorporates various aspects of electronics-shop technical development. The detector was designed to be low-power and extremely portable, which opens up a wide range of physics for students to explore. This document describes the physics behind the Desktop Muon Detectors and explores possible measurements that can be made with the detectors. In particular, we explore various physical phenomena associated with the geomagnetic field, atmospheric conditions, cosmic ray shower composition, attenuation of particles in matter, radioactivity, and statistical properties of Poisson processes.

==> FutureMeasurements.tex <==

\chapter{\textsc{Future measurements}}\label{sec::future}
This section compiles a list of potential future experiments that we intend to perform. After gather and analysing the data, these will be added into Sec.~\ref{sec::measurements}.

\begin{enumerate}
\item \textbf{Muon rate underwater}: Physicists typically report the equivalent overburden in terms of how much water would provide the equivalent shielding. A measurement in actual water can be useful since it provides a homogeneous material and is abundant. We will attempt to measure the attenuation as a function of depth in a deep lake/ocean. Initially, we should observe a steep decrease due to the electromagnetic component dropping out, then a slow decrease as a function of depth. 
\item \textbf{Subway measurement}: Subways are typically buried under a significant amount of concrete and soil. A measurement at different subways could be interesting since it is easily accessible.
\item \textbf{cosmic-ray muon rate at different floors of a large concrete building}: Large concrete buildings, like FermiLab would be great to measure the floor to floor vertical attenuation. 
\item \textbf{Special relativity measurement}: A repeat of the measurement that confirmed special relativity by measuring the muon rate on top and at the bottom of a mountain. This can be demonstrated using the altitude data here; however, climbing a mountain would make a good story.
\item \textbf{Thin lead measurements}. Thin lead sheets, above the coincidence detectors will actually cause an increase in the count rate. This is due to the muon creating a shower of secondaries, that spread out and are able to trigger the detectors simultaneously. After a few inches of lead, the shower is attenuated. 
\item \textbf{Clean room background measurement.} Background measurement in clean room at SNO+, also a coincidence measurement. 
\item \textbf{Measure the Southern Atlantic Anomaly}. This could be performed by flying from Mexico to northern Africa. 
\item \textbf{Extreme weather events}: Measure muon rate during a low pressure event -- like a hurricane.
\item \textbf{Solar flare events}: Capture data during an intense solar flare.
\item \textbf{Solar activity}: There is an 11-year due to the solar activity that modulates the low-energy cosmic rays.
\end{enumerate}


==> Introduction.tex <==

\begin{figure}[h]
\begin{center}
\includegraphics[width=1\columnwidth]{Figures/Intro_sm.png}
\caption{The Standard Model of Particle Physics. Charge is in units of the charge of an electron.}
  \label{fig::sm}
 \end{center}
\end{figure}


\chapter{\textsc{Introduction}}\label{ch:Introduction: a kink in the armour}
The Standard Model (SM) of particle physics is currently the leading fundamental theory of our universe. It reduces everything we see in nature down to a simple set of particles and force carriers. While this theory has been tested to un-imaginable accuracy (see for example the measurements on the electron magnetic moment \cite{}), we (physicist) expect that it cannot be the final level of understanding. The first breaking of the SM picture came in 1996 with the first measurement of neutrino oscillations. Beyond this, we know that this cannot be the final picture; simple questions have yet to be answered: how does gravity fit, what is dark matter and dark energy, . The majority of the particle physics is concerned with attempting to probe the SM theory to the precision that we think it will break down and give us insight into what comes next. The measurement of neutrino oscillation in 1996 was the first successful direct measurement to show that the theory is incomplete. This analysis aims to search for a second kink in the theory -- the search for sterile neutrinos. 

In this thesis, I will often attempt to use natural units in which c = $\hbar$ = 1. 
Section on definitions.


Outline of thesis.

Let's begin.

Nonetheless,
they have rather unique roles in the world of elementary particles. T

\section{The Standard Model of particle physics}
Describe the standard model, how it works. 
The SM is summarized in Fig.~\ref{fig::sm}. Particles are characterized by their mass, spin, and quantum numbers determining their interactions (such as charge). Fermions have spin 1/2, (outlined in green in Fig.~\ref{fig::sm})

Each particle has it's own history and this thesis concentrates on the three neutral leptons known as neutrinos.

In this thesis, I'll be using natural notation. 
The two fundamental constants, viz., the Planck’s constant, hbar, and the velocity of light in vacuum, c, appear
repeatedly in expressions in relativistic quantum mechanics and high energy physics. It is convenient to use a
system of units in which the use of these two constants can be avoided, thereby hugely simplifying such
expressions.

This can be achieved by choosing units hbar = c = 1, where hbar is the reduced Planck’s constant.


\section{The history of neutrinos}
To date all of our knowledge about neutrinos comes from analyzing neutrino data from several sources. From some of these sources, we have but one single measured neutrino (from a Blazar), while others we measured 24 neutrinos withing the course of 5ms, and haven't seen any others since (supernova). In an attempt to study neutrino interactions with high precision, we build neutrino factories (using accelerators). While nature also provides us with a reliable shower of neutrinos know from cosmic-ray interactoins. Neutirnos may also be a portal to probing different particles like Dark matter. They . All of this began in 1930 with a simple observation that the energy spectrum from beta decay was not mono-energetic.

\begin{figure}[!b]
\begin{center}
\includegraphics[width=1.\columnwidth]{Figures/Intro_sources.jpg}
\caption{}
  \label{fig::fit}
 \end{center}
\end{figure}



Describe Pauli -> everything. 
First measurement by reines. 

How do we know it is spin 1/2
How do we know that  it has no charge.
It was used to come up with lepton Number conservation. Which lead to quark number conservation.
Solar neutrino mistery
Lead to mass. 
Other mysteries description, what will they lead to.
Describe the oscillation anomaly, and use it as an analogy to the sterile neutrino hypothesis.  
	
	The Standard Model (SM) of particle physics is currently the leading fundamental theory of our universe. It reduces everything we see in nature down to a simple set of particles (fermions) and bosons (force carrying particles), shown in the above fig.. While this theory has been tested to un-imaginable accuracy, we (physicist) expect that it cannot be the final level of understanding. Neutrino oscillation appears to be the first kink in the theory, where the SM was modified in order to give the neutrinos mass -- something that requires an extension the the SM. Scientists in the future will find that we must also incorporate the Dark Matter ().



==> biblio.tex <==
%% This defines the bibliography file (main.bib) and the bibliography style.
%% If you want to create a bibliography file by hand, change the contents of
%% this file to a `thebibliography' environment.  For more information 
%% see section 4.3 of the LaTeX manual.
\begin{singlespace}
\bibliography{main}
\bibliographystyle{plain}
\end{singlespace}


==> forward.tex <==
% $Log: abstract.tex,v $
% Revision 1.1  93/05/14  14:56:25  starflt
% Initial revision
% 
% Revision 1.1  90/05/04  10:41:01  lwvanels
% Initial revision
% 
%
%% The text of your abstract and nothing else (other than comments) goes here.
%% It will be single-spaced and the rest of the text that is supposed to go on
%% the abstract page will be generated by the abstractpage environment.  This
%% file should be \input (not \include 'd) from cover.tex.


\begin{figure}[!t]
\begin{center}
\includegraphics[width=1.\columnwidth]{Figures/deloyement.jpg}
\caption{The IceCube Lab}
  \label{fig::antarctic}
 \end{center}
\end{figure}



In December 2018, I flew to the South Pole as part of a field team to perform maintenance and upgrades on the IceCube Neutrino Observatory~\cite{icecube}. During the flight I measured the ionizing radiation with two detectors orientated in configuration (d) of Fig.~\ref{fig::opening_angle}. Data was recorded to the microSD cards and powered through a single 30,000~mAh power bank. 

The first four flights (from Madison, WI USA to Christchurch, New Zealand) were operated by United Airlines and New Zealand Airlines. The altitude data was publicly available for these flights on FlightAware.com~\cite{flight_data}.  The flight leaving from Christchurch New Zealand, to McMurdo Antarctica, was on a C-17 military jet operated by the US Air Force. Similarly, we flew on a C-130 Hercules, the day after to the South Pole. Since these were military flights, the altitude of this flight was not available; however, several altitude measurements on the second flight were made using GPS. We landed several days later on the 2700~m thick South Pole glacier, approximately 0.5~km from the actual Geographical South Pole.

The full master and coincident detector data are shown in Fig.~\ref{fig::long_flight}, with descriptions of each flight in the text boxes. To give perspective for other measurements, the total data collected by the master detector was about 50~Mb, whereas the coincidence detector was approximately 15~Mb.


Fig.~\ref{fig::long_flight} illustrates a several very interesting properties. First, there is a trend towards lower count rates near the equator. This is due to the latitudinal variation in the cosmic ray flux described in Sec.~\ref{sec::variations_atm}. This effect is most obvious in the flight from SFO to ACK, which traveled at nearly a constant altitude and a constant rate of latitude change from +32$^\circ$ to -32$^\circ$. We see that the rate is not symmetric. This is because the magnetic latitude is offset from the geographical latitude, which in turn is because the magnetic field is not symmetric about the equator. Second, it's interesting to see that when we landed at the South Pole, there is a noticeable change in trigger rate due to the combination of the elevation and change in Earth's magnetic field.

While flying through the equator at 35,000~ft, I performed an East-West measurement using configuration (e) of Fig.~\ref{fig::opening_angle}. We measure a count rate coming from the east of 0.69~+/-~0.02~cps, while from the west 0.84~+/- 0.03~cps. This represents a 22.2$\pm$7.4\% increase in the westward direction. This east-west asymmetry is described in Sec.~\ref{sec::variations_atm}.


\begin{figure}[!t]
\begin{center}
\includegraphics[width=1.\columnwidth]{Figures/sp.jpg}
\caption{The IceCube Lab}
  \label{fig::antarctic}
 \end{center}
\end{figure}
